Mapping Spiking Neural Networks to Heterogeneous Crossbar Architectures using Integer Linear Programming

Advances in novel hardware devices and architectures allow Spiking Neural Network evaluation using ultra-low power, mixed-signal, memristor crossbar arrays. As individual network sizes quickly scale beyond the dimensional capabilities of single crossbars, networks must be mapped onto multiple crossbars. Crossbar sizes within modern Memristor Crossbar Architectures are determined predominately not by device technology but by network topology; more, smaller crossbars consume less area thanks to the high structural sparsity found in larger, brain-inspired SNNs. Motivated by continuing increases in SNN sparsity due to improvements in training methods, we propose utilizing heterogeneous crossbar sizes to further reduce area consumption. This approach was previously unachievable as prior compiler studies only explored solutions targeting homogeneous MCAs. Our work improves on the state-of-the-art by providing Integer Linear Programming formulations supporting arbitrarily heterogeneous architectures. By modeling axonal interactions between neurons our methods produce better mappings while removing inhibitive a priori knowledge requirements. We first show a 16.7-27.6% reduction in area consumption for square-crossbar homogeneous architectures. Then, we demonstrate 66.9-72.7% further reduction when using a reasonable configuration of heterogeneous crossbar dimensions. Next, we present a new optimization formulation capable of minimizing the number of inter-crossbar routes. When applied to solutions already near-optimal in area an 11.9-26.4% routing reduction is observed without impacting area consumption. Finally, we present a profile-guided optimization capable of minimizing the number of runtime spikes between crossbars. Compared to the best-area-then-route optimized solutions we observe a further 0.5-14.8% inter-crossbar spike reduction while requiring 1-3 orders of magnitude less solver time.

==> figures/experiments/breakdown_figure_2.tex <==
% This figure is placed in its own file so that we can move it around
% in the text more easily. Because it's a double-column figure, we must take extra
% care to place it in the right place.



% Tex hacking:
\makeatletter
% \markbb{prefix}{content}
%
% Sets tikzmarks at the bounding box corners of `content'
%
% Tikzmarks are prefixed by `prefix'. For example, Setting prefix to Lastbox
% would create the tikzmarks Lastbox_NW, Lastbox_NE, Lastbox_SW, and Lastbox_SE
%
\newcommand{\markbb}[2]{
\tcbset{markbbstyle/.style={enhanced, boxsep=0pt, left=0pt, right=0pt, top=0pt,
                            bottom=0pt, arc=0pt,
                            boxrule=0pt, toprule=0pt,
                            sharp corners, frame hidden,
                            colback=white,
                            overlay={
                                \begin{scope}
                                    \draw (frame.north west) node {\tikzmark{#1_NW}};
                                    \draw (frame.north east) node {\tikzmark{#1_NE}};
                                    \draw (frame.south west) node {\tikzmark{#1_SW}};
                                    \draw (frame.south east) node {\tikzmark{#1_SE}};
                                \end{scope}
                                }
                            }
}
\begin{tcolorbox}[markbbstyle]
#2
\end{tcolorbox}}
\makeatother

% And it's used as thus:
\begin{figure*}[t]
    \centering
    \begin{minipage}{0.38\linewidth}
        \begin{subfigure}{\linewidth}
            \markbb{BP1}{
                \centering
                \includesvg[width=\textwidth]{figures/experiments/het_breakdown/out-109-axsh.svg}
                \caption{Network A Breakdown}
                \label{subfig:breakdown-main}
            }
        \end{subfigure}
    \end{minipage}
    \hfill
    \begin{minipage}{0.6\linewidth}
        \captionsetup[subfigure]{aboveskip=0.049cm}
        \begin{subfigure}{\linewidth}
            \markbb{BP2}{
                \centering
                \includesvg[width=\textwidth]{figures/experiments/het_breakdown/out-bar.svg}
                \caption{Makeup Per Net}
                \label{subfig:bs-1}
            }
        \end{subfigure}
        \\
        \vspace{-0.28em}
        
        \begin{subfigure}{\linewidth}
            \markbb{BP6}{
                \centering
                \hspace{-2.51em}
                \setlength{\tabcolsep}{3pt}
                \renewcommand{\arraystretch}{0.93}
                \setlength\tabcolsep{1pt}
                \begin{tabular}{| l | l | l | l | l | l | l |}
                    \hline
                    Network & Best Solution & Break-Even    & \multicolumn{4}{c|}{Crossbar Count/Contribution\%} \\
                    \cline{4-7}
                            & Time (s, det) & Time (s, det) & 4x4 & 8x4 & 16x4 & 32x4 \\
                    \hline
                    A & 87432  & 59.4 & 31/30.1\% & 20/38.8\% & 6/23.3\%  & 1/7.8\%\\
                    B & 1637   & 27.7 & 32/30.2\% & 31/58.5\% & 1/3.8\%   & 1/7.5\%\\
                    C & 122225 & 27.3 & 14/15.2\% & 11/23.9\% & 10/43.5\% & 2/17.4\%\\
                    D & 71402  & 63.2 & 32/29.1\% & 25/45.5\% & 7/25.5\%  & 0/0.0\%\\
                    E & 91257  & 17.0 & 15/17.2\% & 10/23.0\% & 13/59.8\% & 0/0.0\%\\
                    \hline
                \end{tabular}
                \vspace{0.5em}
                \caption{Summary}
                \label{fig:sb-summary}
            }
        \end{subfigure}
    \end{minipage}

    
    \begin{tikzpicture}[remember picture, overlay]

        \draw (pic cs:BP2_SE) ++ (0.1, -0.1) coordinate (midsep);
        \draw (pic cs:BP2_NE) ++ (0.25, 0.15) ++ (-7.725, 0) coordinate (figNE);

        % Tikzmarks are weird so we must define complex coordinates like this        
        \path let \p1=(pic cs:BP1_NW),\p2=(figNE) in coordinate (pathstart) at (\x1, {max(\y1,\y2)});
        \path let \p1=(pic cs:BP2_SW),\p2=(midsep) in coordinate (right_join) at (\x1, \y2);
        \path let \p1=(right_join),\p2=(pic cs:BP1_SE) in coordinate (mid_join) at (\x2, \y1);
        \path let \p1=(pathstart),\p2=(midsep) in coordinate (topright) at (\x2, \y1);

        \draw[red, dashed]
        (pathstart)
        -- (figNE)%(topright)
        -- (midsep -| figNE)
        -- (mid_join)
        -- (pic cs:BP1_SE)
        -- (pic cs:BP1_SW)
        -- (pathstart);
    \end{tikzpicture}

    \captionsetup{format=hang}
    \caption{Area optimization targeting reasonable heterogeneous architecture\\
    The ILP solver did not terminate for these tasks; the best solutions found within a 5 hour limit are reported
    }
    \label{fig:breakdown}

    \vspace*{-1\baselineskip} % IEEETran puts WAY too much padding around figures
\end{figure*}

==> preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Preamble
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Encodings
% Use utf8 encoding for the input file and T1 font encoding.
\usepackage[utf8]{inputenc}  % Specify the file input encoding.
\usepackage[T1]{fontenc}     % Specify to use T1 font encoding.

%%% PAGE DIMENSIONS
\usepackage{geometry}  % to change the page dimensions
\geometry{letterpaper} % or letterpaper (US) or a5paper or....
\geometry{margin=1in}  % for example, change the margins to 2 inches all round

%%% PACKAGES
% Add support for url typesetting
%\usepackage[hyphens]{url}

% Use biblatex with the biber backend.
% \usepackage[backend=biber,citestyle=ieee]{biblatex}

% Used to fit the bibliography within the margins. Without this, you will get
% overfull hbox warnings.
%\usepackage[final,nopatch=footnote]{microtype}

% Specify the bib file to include.
% \addbibresource{references.bib}

% Specify colors
%\usepackage[table]{xcolor}

% Allows specifying counters and performing math on lengths
\usepackage{calc}

% Add verbatim environment
\usepackage{verbatim}

% Use the graphicx package in pdf mode to include images into the document.
%\usepackage[pdftex]{graphicx}
\usepackage[]{graphicx}

% Add additional mathematical typesetting commands.
\usepackage{amsmath, amssymb, amsthm, amstext, amsopn, amsfonts}

% Math formatting tools.
\usepackage{IEEEtrantools}

% Adds additional options for the array and tabular environments.
\usepackage{array}

% Add additional options for floats
\usepackage{float}

% Add additional enumeration commands
\usepackage[inline]{enumitem}

% Allows figures to be broken down in to subfigures.
\usepackage[caption=false,font=footnotesize]{subfig}

% Add support for typesetting units.
\usepackage{siunitx}

% Add support for hyperlinks in the PDF. Do not let the hyperlinks show up.
%\usepackage[hidelinks]{hyperref}

% Support for adding code blocks
\usepackage{listings}

% Plotting library for creating graphs.
\usepackage{pgfplots}

% Dummy text for format testing
\usepackage{lipsum}

% Support author blocks
\usepackage{authblk}

% Indent first paragraph
\usepackage{indentfirst}

% Todo notes
\usepackage[colorinlistoftodos,prependcaption,textsize=footnotesize,color=limeyellow,linecolor=magenta]{todonotes}
\usepackage{hyperref}

% Set spacing
\usepackage{setspace}

% Layout manipulation
\usepackage{xspace}

% Specify the directories for storing images.
\graphicspath{{figures/}{inkscape/}}

% Set the version of pgfplot to the latest version.
\pgfplotsset{compat=newest}

% Correct bad hyphenation here
% \hyphenation{}

% Remove page group warnings caused by pdflatex
\pdfsuppresswarningpagegroup=1

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Helper Commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% These helper commands specify consistent ways of referencing various document
% parts.
\makeatletter
\newcommand*{\reffigure}{\@ifstar{\@reffigures}{\@reffigure}}
\newcommand*{\@reffigure}[1]{\hyperref[#1]{Figure~}\ref{#1}}
\newcommand*{\@reffigures}[1]{\hyperref[#1]{Figures~}\ref{#1}}
\newcommand*{\reftable}{\@ifstar{\@reftables}{\@reftable}}
\newcommand*{\@reftable}[1]{\hyperref[#1]{Table~}\ref{#1}}
\newcommand*{\@reftables}[1]{\hyperref[#1]{Tables~}\ref{#1}}
\makeatother
\newcommand*{\refchapter}[1]{\hyperref[#1]{Chapter~}\ref{#1}}
\newcommand*{\refappendix}[1]{\hyperref[#1]{Appendix~}\ref{#1}}
\newcommand*{\refsection}[1]{\hyperref[#1]{Section~}\ref{#1}}
\newcommand*{\refsubsection}[1]{\hyperref[#1]{Subsection~}\ref{#1}}
\newcommand*{\refalgorithm}[1]{\hyperref[#1]{Algorithm~}\ref{#1}}
\newcommand*{\refequation}[1]{\hyperref[#1]{Equation~}\ref{#1}}


